A Morphology Focused Diffusion Probabilistic Model for Synthesis of Histopathology Images

Visual microscopic study of diseased tissue by pathologists has been the cornerstone for cancer diagnosis and prognostication for more than a century. Recently, deep learning methods have made significant advances in the analysis and classification of tissue images. However, there has been limited work on the utility of such models in generating histopathology images. These synthetic images have several applications in pathology including utilities in education, proficiency testing, privacy, and data sharing. Recently, diffusion probabilistic models were introduced to generate high quality images. Here, for the first time, we investigate the potential use of such models along with prioritized morphology weighting and color normalization to synthesize high quality histopathology images of brain cancer. Our detailed results show that diffusion probabilistic models are capable of synthesizing a wide range of histopathology images and have superior performance compared to generative adversarial networks.

==> Discussion.tex <==
\section{Discussion}\label{sec:discussion}
% visual quality from Sanne
\begin{figure}[tp]
\begin{center}
    \includegraphics[scale=.84]{figs/FailedCasesProGAN.pdf}
    \caption{Examples of failed cases generated by ProGAN }
    \label{fig:ModeCollapse}
\end{center}
\end{figure}

%\subsection{Visual Observation:}
$The bottom row in \autoref{fig:good-generated-images} shows the images generated by our diffusion model. In these images, cell nuclei stained by purplish blue and extracellular matrix and cytoplasm stained by pink color related to H$\&$E staining, which suggests that using the color normalization module is effective.
Although medical inspection of generated images should be done by pathologists, there are some well known histology features in LGG images that can be identified even by an untrained person. The so-called "fried egg" appearance~\cite{OligoPattern} of oligodendrogliomas is shown in the synthetic images (such as the bottom first and second images in~\autoref{fig:good-generated-images}, top second image or bottom fourth image at~\autoref{fig:Top10} in the supplementary material), namely in the IDHC and IDHWT. Another characteristic of the oligodendrogliomas that can be seen in generated images by diffusion (such as the bottom second column of~\autoref{fig:good-generated-images}) is branching small, chicken wire-like blood vessels~\cite{OligoPattern}, and this characteristic can also be found in the IDHC. This suggests that the diffusion model was able to learn specific known histopahological features. However, these accurate features do not clearly exist in the images generated by ProGAN. In addition, the IDHWT are the most uncommon among the other two, and it appears that the lesser number of cases for the IDHWT subtype resulted in artefacts and lower image quality of ProGAN as compared to the diffusion, implying that ProGAN got stuck in mode collapse (\autoref{fig:ModeCollapse}) due to a lack of enough data points in this subtype. However, the diffusion could learn these rare class specific features.  \autoref{fig:ModeCollapse} shows samples of failed images by ProGAN in which each image is produced from random noise; however, they are fairly similar to each other.

%\subsection{Numerical Observation:}
%Visual observations match with objective metrics presented in~\autoref{tab:Exp1_set1} and~\autoref{tab:Exp1_set2}. A better FID, sFID, and Improved Precision show the superiority of the diffusion model over ProGAN in generating high quality and fidelity samples. On the other hand, a significant GAP between reported Improved Recall values in 
%\autoref{tab:Exp1_set2} means better diversity and distribution coverage of the produced images by diffusion model compared to ProGAN. The lower diversity of ProGAN generated images has shown its effect in mode collapse and generating similar images in \autoref{fig:ModeCollapse}.
%Although the results from experiment II show the similarity of the morphological features of synthetic and real images, the differences between each pathologists opinions comes from their various level of experience. Compared to P2, the first pathologist(P1), with the most expertise, was more confident regarding his decisions and detected most real images correctly. He also could not distinguish more than 82\% of synthesized images(classified them with high confidence as real), and he had medium confidence for most of the cases that he correctly detected as synthetic. On the other hand, P2 with lower experience faced more serious difficulty in distinguishing synthetic images from the real ones. Also, by using two sided Fisher-exact test, we observed that pathologists' observations for the real and synthetic images are not statistically different. Therefore, our survey's results indicate the high quality and similarity of the synthetic and real images in terms of morphological features. 


%\subsection{Future Works}
%The work in this paper can be extended by optimizing the proposed model to reduce diffusion probabilistic models sampling time since it is relatively longer than GANs due to multiple small diffusion steps. As an instance, this work can be extended by benefiting from Xiao et al.~\cite{vahdat-problem} work that uses a multimodal conditioned  discriminator following the diffusion model and can considerably reduce the number of diffusion steps.

